The implementation of a broad class of boundary conditions for non-linear hyperbolic systems

We propose methods that augment existing numerical schemes for the simulation of hyperbolic balance laws with Dirichlet boundary conditions to allow for the simulation of a broad class of differential algebraic conditions. Our approach is similar to that of Thompson (1987), where the boundary values were simulated by combining characteristic equations with the time derivative of the algebraic conditions, but differs in two important regards. Firstly, when the boundary is a characteristic of one of the fields Thompson's method can fail to produce reasonable values. We propose a method of combining the characteristic equations with extrapolation which ensures convergence. Secondly, the application of algebraic conditions can suffer from $O(1)$ drift-off error, and we discuss projective time-stepping algorithms designed to converge for this type of system. Test problems for the shallow water equations are presented to demonstrate the result of simulating with and without the modifications discussed, illustrating their necessity for certain problems.

==> Sections/ExtrapCondn.tex <==
\section{Conditions on extrapolation and differentiation} \label{sec:ExtrapCondn}

To justify constraints on coefficients use
\begin{align}
	\hat{\Gamma} &\eqdef \sum_j \hat{\gamma}_j Q_j = \sum_j \hat{\gamma}_j \cdot \ppar*{ Q_R + \frac{Q_j - Q_R}{x_j - x_R} (x_j - x_R) }
	&\text{where}&&
	\frac{Q_j - Q_R}{x_j - x_R} = \eval*{\pdv{Q}{x}}_{x=x_R} + \order{ \Delta x },
\end{align}
the $\order{ \Delta x }$ correction terms depending on whether $Q_j$ represent the values at points (finite differencing) or averaged across volumes (finite volume) ($Q_R$ always represents the value at the point $x=x_R$). Thus
\begin{equation}
	\hat{\Gamma} = Q_R \sum_j \hat{\gamma_j} + \eval*{\pdv{Q}{x}}_{x=x_R} \sum_j \hat{\gamma}_j (x_j - x_R) + \order{(\Delta x)^2}
\end{equation}
which gives the constraints on the coefficients for the sum to represent the value or derivative at $x=x_R$. 

==> Templates/StandardMathsMacros.tex <==
%My macros for the math environment

\usepackage{xparse}
\makeatletter




%---BRACKETS----

%Normal brackets

\DeclarePairedDelimiter{\ppar}{\lparen}{\rparen}
\DeclarePairedDelimiter{\pang}{\langle}{\rangle}
\DeclarePairedDelimiter{\pbrc}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\pbrk}{\lbrack}{\rbrack}
\DeclarePairedDelimiter{\pgrp}{\lgroup}{\rgroup}

%Bracket-like structures

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\round}{\lfloor}{\rceil}

\DeclarePairedDelimiter{\eval@wdot}{.}{\rvert}
\NewDocumentCommand{\eval}{som}{%
	\IfBooleanTF{#1}
    	{\eval@wdot*{#3}}
   		{\IfNoValueTF{#2}{#3\rvert}{\eval@wdot[#2]{#3}}}%
}

\DeclarePairedDelimiterX{\setpred}[2]{\lbrace}{\rbrace}{\: #1 \: \delimsize\vert \: #2 \:}




%---OPERATORS---

\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\minmod}{minmod}
\DeclareMathOperator{\diag}{diag}




%---DIMENSIONLESS CONSTANTS---
%Define carefully, some of these are defined in the JFM template

%\Rey Reynolds number 
\ifdefined\Rey\else
	\newcommand\Rey{\mbox{\textit{Re}}}
\fi

%\Pran Prandtl number
\ifdefined\Pran\else
	\newcommand\Pran{\mbox{\textit{Pr}}} 
\fi

%\Pen Peclet number
\ifdefined\Pen\else
	\newcommand\Pen{\mbox{\textit{Pe}}}
\fi

%\Fro Froude number
\ifdefined\Fro\else
	\newcommand\Fro{\mbox{\textit{Fr}}}
\fi

%\Ric Richardson number
\ifdefined\Ric\else
	\newcommand\Ric{\mbox{\textit{Ri}}}
\fi




%---CALCULUS---
%Uses the calculus syntax from the Physics package with a few modifications
%
%For fractions p/q, following applies
%\frac{p}{q}, standard
%\frac*{p}{q}, flat
%\frac**{p}{q}, flat, autosize slash
%\frac*[\size]{p}{q}, flat, slash size of \size
%
%For differential d syntax is
%\dd*[power]{measure}
%Star removes spacing
%
%For derivative df/dx, stars the same as for \frac, optional argument the order of the derivative
%\dv(frac syntax here)[order]{f}{x}
%If wanting to use a flat derivative without sizing with order, then \dv*[][n]{f}{x}
%
%For partial derivative df/dx, use \pdv with syntax as for \dv
%NOT IMPLEMENTED YET Alternatively, for d^n f/dx_1 ... dx_n use
%\pdvm(frac syntax here){n}{f}{x_1}...{x_n}

%\frac
\let\frac@nostar\frac
\DeclarePairedDelimiterX{\frac@starwdot}[2]{.}{.}{#1 \delimsize/ #2}
\NewDocumentCommand{\frac@star}{somm}{%
	\IfBooleanTF{#1}
    	{\frac@starwdot*{#3}{#4}}
    	{\IfNoValueTF{#2}{#3/#4}{\frac@starwdot[#2]{#3}{#4}}}%
}
\renewcommand*\frac{\@ifstar{\frac@star}{\frac@nostar}}

%\dd
\NewDocumentCommand{\dd}{som}{%
	\IfBooleanF{#1}{\,}%
	\IfNoValueTF{#2}{%Check whether optional argument is given
		\textrm{d} #3%
	}{%
		\textrm{d}^{#2} #3%
	}%
	\IfBooleanF{#1}{\,}%
}

%\dv
\NewDocumentCommand\dv@nostar{O{}mm}{%
	\frac@nostar{\textrm{d}^{#1} #2}{{\textrm{d} #3}^{#1}}
}
\NewDocumentCommand{\dv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\textrm{d}^{#2} #4}{{\textrm{d} #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\textrm{d}^{#3} #4}{{\textrm{d} #5}^{#3}}%
		\else
			\frac*[#2]{\textrm{d}^{#3} #4}{{\textrm{d} #5}^{#3}}%
		\fi
	}%
}
\newcommand*\dv{\@ifstar{\dv@star}{\dv@nostar}}

%\pdv
\NewDocumentCommand\pdv@nostar{O{}mm}{%
	\frac@nostar{\partial^{#1} #2}{{\partial #3}^{#1}}
}
\NewDocumentCommand{\pdv@star}{sO{}O{}mm}{%
	\IfBooleanTF{#1}{%
		\frac**{\partial^{#2} #4}{{\partial #5}^{#2}}%
	}{%
		\if \relax\detokenize{#2}\relax
			\frac*{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\else
			\frac*[#2]{\partial^{#3} #4}{{\partial #5}^{#3}}%
		\fi
	}%
}
\newcommand*\pdv{\@ifstar{\pdv@star}{\pdv@nostar}}

%%\pdvm
%\NewDocumentCommand\pdvm@nostar@two{mmmm}{%
%	\frac{\partial^2 #2}{\partial #3 \partial #4}
%}
%\NewDocumentCommand{\pdvm@star@two}{sO{}mmm}{%
%	|#1,#2,#3,#4,#5|
%%	\IfBooleanTF{#2}{%
%%		\frac**{\partial^2 #4}{\partial #5 \partial #6}%
%%	}{%
%%		\if \relax\detokenize{#3}\relax
%%			\frac*{\partial^2 #4}{\partial #5 \partial #6}%
%%		\else
%%			\frac*[#3]{\partial^2 #4}{\partial #5 \partial #6}%
%%		\fi
%%	}%
%}
%\newcommand*\pdvm@nostar[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm@STAR[1]{%
%	\ifnum #1=2
%		\pdvm@nostar@two%
%	\fi%
%}
%\newcommand*\pdvm{\@ifstar{\pdvm@star}{\pdvm@nostar}}

%\def\pdvm@str@frac{frac}
%\def\pdvm@str@flat{flat}
%\def\pdvm@str@slsh{slsh}
%
%\NewDocumentCommand{\pdvm@two}{mmmmm}{
%	F|#1,#2,#3,#4,#5|
%}
%
%\newcommand*\pdvm@nostar[1]{%
%	A|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@frac}{}%
%	\fi%
%}
%\newcommand*\pdvm@star[2]{%
%	B%\abs{ #1 , #2 } \:
%%	\ifnum #2=2
%%		\pdvm@two{\pdvm@str@slsh}{#1}%
%%	\fi%
%}
%\newcommand*\pdvm@sstar[1]{%
%	C|#1| \:
%	\ifnum #1=2
%		\pdvm@two{\pdvm@str@flat}{}%
%	\fi%
%}
%
%\newcommand\pdvm@staropt[1][]{%
%	a| #1 | \:%
%	\if \relax\detokenize{#1}\relax
%		b%
%		\pdvm@star{}%
%	\else
%		c%
%		\pdvm@star{#1}%
%	\fi
%}
%\newcommand*\pdvm@STAR{\@ifstar{\pdvm@sstar}{\pdvm@staropt}}
%\newcommand*\pdvm{\@ifstar{\pdvm@STAR}{\pdvm@nostar}}


%---ORDER NOTATION---

%If order is used with an empty argument then dont use parenthesis
\newcommand{\order@text}[1]{	
	\if\relax\detokenize{#1}\relax% #1 is empty
	\else% #1 is nonempty
		\ppar*{#1}%\qty(#1)
	\fi
}

%Big O
\newcommand{\order}[1]{
	\mathcal{O}\order@text{#1}
}

%Little O
\newcommand{\lorder}[1]{
  	\mathchoice
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \displaystyle
    	{{\scriptstyle\mathcal{O}}\order@text{#1}}% \textstyle
    	{{\scriptscriptstyle\mathcal{O}}\order@text{#1}}% \scriptstyle
    	{\scalebox{.6}{${\scriptscriptstyle\mathcal{O}}\order@text{#1}$}}%\scriptscriptstyle
  	}

%Big Theta
\newcommand{\Torder}[1]{
	\mathit{\Theta}\order@text{#1}
}




%---ASSORTED---

%Have equation span full width of collumn (good for equations in lists)
\newcommand{\eqnwide}{\displayindent0pt \displaywidth\textwidth}

%Use as 10^\nth
\newcommand{\nth}{\text{th}}

%Defined to be equal to
\newcommand{\eqdef}{\vcentcolon =}%{\stackrel{\mathrm{def}}{=}}

%Text style fraction
\newcommand{\textfrac}[2] {{\textstyle\frac{#1}{#2}}}

%Omitted dummy variable as a dot
\newcommand*\omitdummy{\mathchoice
	{\omitdummy@{\displaystyle}{0.6}}
	{\omitdummy@{\textstyle}{0.6}}
	{\omitdummy@{\scriptstyle}{0.7}}
	{\omitdummy@{\scriptscriptstyle}{0.8}}
}
\newcommand*\omitdummy@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}




%---ENVIRONMENTS---

%Like cases but with as many collumns as you like

\newenvironment{multicasesnobrac}[1][1]{%
%No braces
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}
}
\newenvironment{multicases}[1][1]{%
%Left braced
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{r@{}l}}
}{
	\end{array}\right.
}
\newenvironment{multicasesd}[1][1]{%
%Left braced with display style
%#1 	number of equations in horizontal direction, by deafualt 1
	%
	\left\{\begin{array}{*{#1}{>{\displaystyle}{r}@{}>{\displaystyle}{l}}}
}{
	\end{array}\right.
}




%---SIDE BY SIDE SUBEQUATIONS---

%Multiple labeled equations on same line
\newlength{\sbsse@Wl}	%Width of left equation
\newlength{\sbsse@Wm}	%Width of mid text
\newlength{\sbsse@Wr}	%Width of right equation
\newlength{\sbsse@Wt}	%Width of tag
\newlength{\sbsse@We}	%Remaining width on line
\newlength{\sbsse@Wd}	%Remaining width divided into pieces

%Two equations side by side
\newcommand\sidebysidesubequations[6]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    midtext
	% #5    right subequation
	% #6    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{\text{#4}}
	\def\sbsse@Er{#5}
	\def\sbsse@Et{(\ref*{#1}a,b)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space, and midtext if any
			\if\relax\detokenize{#4}\relax
				\setlength{\sbsse@Wd}{\sbsse@We/3}
				\hspace{\sbsse@Wd}
			\else
				\setlength{\sbsse@Wd}{\sbsse@We/4}
				\hspace{\sbsse@Wd}\sbsse@Em\hspace{\sbsse@Wd}
			\fi
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#6}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}

%Three equations side by side
\newcommand\sidebysidesubequationsT[7]{%
	% #1    reference label
	% #2    left subequation
	% #3    left label
	% #4    mid subequation
	% #5	mid label
	% #6    right subequation
	% #7    right label
  
	%Setup the equations to be typed
	\def\sbsse@El{#2}
	\def\sbsse@Em{#4}
	\def\sbsse@Er{#6}
	\def\sbsse@Et{(\ref*{#1}a,b,c)}
	%Compute the widths
	\settowidth{\sbsse@Wl}{\begin{math}\displaystyle\sbsse@El\end{math}}
	\settowidth{\sbsse@Wm}{\begin{math}\displaystyle\sbsse@Em\end{math}}
	\settowidth{\sbsse@Wr}{\begin{math}\displaystyle\sbsse@Er\end{math}}
	\settowidth{\sbsse@Wt}{\sbsse@Et}
	\setlength{\sbsse@We}{\linewidth-\sbsse@Wl-\sbsse@Wm-\sbsse@Wr-\sbsse@Wt}
	\setlength{\sbsse@Wd}{\sbsse@We/4}
	
	%Begin equation typesetting, with label for overall subequations
	\begin{subequations}\ltx@label{{#1}}
		\begin{displaymath}
			%Left equation and label
			\sbsse@El\refstepcounter{equation}\ltx@label{{#3}}
			%Space
			\hspace{\sbsse@Wd}
			%Mid equation and label
			\sbsse@Em\refstepcounter{equation}\ltx@label{{#5}}
			%Space
			\hspace{\sbsse@Wd}
			%Right equation and label
			\sbsse@Er\refstepcounter{equation}\ltx@label{{#7}}
			%Tag
			\tag*{\sbsse@Et}
		\end{displaymath}
	\end{subequations}
}




\makeatother
